Electrical conductivity of warm neutron star crust in magnetic fields: Neutron-drip regime

We compute the anisotropic electrical conductivity tensor of the inner crust of a compact star at non-zero temperature by extending a previous work on the conductivity of the outer crust. The physical scenarios, where such crust is formed, involve proto-neutron stars born in supernova explosions, binary neutron star mergers and accreting neutron stars. The temperature-density range studied covers the transition from a non-degenerate to a highly degenerate electron gas and assumes that the nuclei form a liquid, i.e., the temperature is above the melting temperature of the lattice of nuclei. The electronic transition probabilities include (a) the dynamical screening of electron-ion interaction in the hard-thermal-loop approximation for the QED plasma, (b) the correlations of the ionic component in a one-component plasma, and (c) finite nuclear size effects. The conductivity tensor is obtained from the Boltzmann kinetic equation in relaxation time approximation accounting for the anisotropies introduced by a magnetic field. The sensitivity of the results towards the matter composition of the inner crust is explored by using several compositions of the inner crust which were obtained using different nuclear interactions and methods of solving the many-body problem. The standard deviation of relaxation time and components of the conductivity tensor from the average are below $\le 10\%$ except close to crust-core transition, where non-spherical nuclear structures are expected. Our results can be used in dissipative magneto-hydrodynamics (MHD) simulations of warm compact stars.

==> sigma_tables.tex <==
%\documentclass[prc,preprint]{revtex4}
%\usepackage{array,rotating,isotope}
%\begin{document}
\newpage
\section*{Supplemental material}
\begin{table}
\begin{center}
\caption {Model NV at $B_{12}=100$} \label{tab:sigma_1}
\vskip 0.2cm
{\scriptsize
\begin{tabular}{ c | c c c c c | c c c c c }
\hline
&  &  &  $T$ = 1 MeV  &  &  &  &  &  $T$ = 5 MeV  &  &  \\ 
\hline
$\log\rho$ & $\log\tau$ & $\omega_c\tau$ & $\log\sigma$ & $\log\sigma_0$ & $\log\sigma_1$ & $\log\tau$ & $\omega_c\tau$ & $\log\sigma$ & $\log\sigma_0$ & $\log\sigma_1$ \\ 
\hline
\hspace{0.05cm} 11.669 \hspace{0.05cm}  &  \hspace{0.05cm} -19.461 \hspace{0.3cm}  &  1.289  &  22.062  &  21.635 \hspace{0.3cm}  &  21.747 \hspace{0.05cm}  &  \hspace{0.05cm} -19.511 \hspace{0.3cm}  &  1.148  &  22.059  &  21.634 \hspace{0.3cm}  &  21.740 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 11.825 \hspace{0.05cm}  &  \hspace{0.05cm} -19.482 \hspace{0.3cm}  &  1.128  &  22.115  &  21.757 \hspace{0.3cm}  &  21.810 \hspace{0.05cm}  &  \hspace{0.05cm} -19.532 \hspace{0.3cm}  &  1.005  &  22.108  &  21.754 \hspace{0.3cm}  &  21.800 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.001 \hspace{0.05cm}  &  \hspace{0.05cm} -19.491 \hspace{0.3cm}  &  1.039  &  22.158  &  21.839 \hspace{0.3cm}  &  21.857 \hspace{0.05cm}  &  \hspace{0.05cm} -19.542 \hspace{0.3cm}  &  0.925  &  22.150  &  21.836 \hspace{0.3cm}  &  21.844 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.167 \hspace{0.05cm}  &  \hspace{0.05cm} -19.491 \hspace{0.3cm}  &  0.994  &  22.198  &  21.898 \hspace{0.3cm}  &  21.897 \hspace{0.05cm}  &  \hspace{0.05cm} -19.542 \hspace{0.3cm}  &  0.883  &  22.188  &  21.894 \hspace{0.3cm}  &  21.882 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.425 \hspace{0.05cm}  &  \hspace{0.05cm} -19.497 \hspace{0.3cm}  &  0.934  &  22.234  &  21.961 \hspace{0.3cm}  &  21.932 \hspace{0.05cm}  &  \hspace{0.05cm} -19.549 \hspace{0.3cm}  &  0.829  &  22.222  &  21.956 \hspace{0.3cm}  &  21.915 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.795 \hspace{0.05cm}  &  \hspace{0.05cm} -19.632 \hspace{0.3cm}  &  0.592  &  22.224  &  22.093 \hspace{0.3cm}  &  21.867 \hspace{0.05cm}  &  \hspace{0.05cm} -19.672 \hspace{0.3cm}  &  0.540  &  22.219  &  22.087 \hspace{0.3cm}  &  21.858 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.985 \hspace{0.05cm}  &  \hspace{0.05cm} -19.624 \hspace{0.3cm}  &  0.547  &  22.316  &  22.202 \hspace{0.3cm}  &  21.941 \hspace{0.05cm}  &  \hspace{0.05cm} -19.665 \hspace{0.3cm}  &  0.498  &  22.306  &  22.192 \hspace{0.3cm}  &  21.925 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.173 \hspace{0.05cm}  &  \hspace{0.05cm} -19.620 \hspace{0.3cm}  &  0.512  &  22.387  &  22.285 \hspace{0.3cm}  &  21.996 \hspace{0.05cm}  &  \hspace{0.05cm} -19.662 \hspace{0.3cm}  &  0.464  &  22.372  &  22.274 \hspace{0.3cm}  &  21.973 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.533 \hspace{0.05cm}  &  \hspace{0.05cm} -19.579 \hspace{0.3cm}  &  0.469  &  22.584  &  22.497 \hspace{0.3cm}  &  22.169 \hspace{0.05cm}  &  \hspace{0.05cm} -19.627 \hspace{0.3cm}  &  0.420  &  22.557  &  22.477 \hspace{0.3cm}  &  22.127 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.900 \hspace{0.05cm}  &  \hspace{0.05cm} -19.105 \hspace{0.3cm}  &  1.070  &  23.290  &  22.959 \hspace{0.3cm}  &  22.988 \hspace{0.05cm}  &  \hspace{0.05cm} -19.237 \hspace{0.3cm}  &  0.790  &  23.172  &  22.948 \hspace{0.3cm}  &  22.860 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 14.120 \hspace{0.05cm}  &  \hspace{0.05cm} -18.364 \hspace{0.3cm}  &  4.654  &  24.236  &  22.880 \hspace{0.3cm}  &  23.548 \hspace{0.05cm}  &  \hspace{0.05cm} -18.767 \hspace{0.3cm}  &  1.838  &  23.841  &  23.186 \hspace{0.3cm}  &  23.458 \hspace{0.05cm}  \\ 
\hline
\end{tabular}
} 
\end{center}
\end{table}
%-
\begin{table}
\begin{center}
\caption {Model D1M at $B_{12}=100$} \label{tab:sigma_1}
\vskip 0.2cm
{\scriptsize
\begin{tabular}{ c | c c c c c | c c c c c }
\hline
&  &  &  $T$ = 1 MeV  &  &  &  &  &  $T$ = 5 MeV  &  &  \\ 
\hline
$\log\rho$ & $\log\tau$ & $\omega_c\tau$ & $\log\sigma$ & $\log\sigma_0$ & $\log\sigma_1$ & $\log\tau$ & $\omega_c\tau$ & $\log\sigma$ & $\log\sigma_0$ & $\log\sigma_1$ \\ 
\hline
\hspace{0.05cm} 11.825 \hspace{0.05cm}  &  \hspace{0.05cm} -19.421 \hspace{0.3cm}  &  1.285  &  22.186  &  21.759 \hspace{0.3cm}  &  21.870 \hspace{0.05cm}  &  \hspace{0.05cm} -19.477 \hspace{0.3cm}  &  1.128  &  22.182  &  21.757 \hspace{0.3cm}  &  21.861 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.001 \hspace{0.05cm}  &  \hspace{0.05cm} -19.424 \hspace{0.3cm}  &  1.223  &  22.219  &  21.819 \hspace{0.3cm}  &  21.908 \hspace{0.05cm}  &  \hspace{0.05cm} -19.481 \hspace{0.3cm}  &  1.071  &  22.212  &  21.817 \hspace{0.3cm}  &  21.897 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.167 \hspace{0.05cm}  &  \hspace{0.05cm} -19.427 \hspace{0.3cm}  &  1.162  &  22.255  &  21.882 \hspace{0.3cm}  &  21.949 \hspace{0.05cm}  &  \hspace{0.05cm} -19.485 \hspace{0.3cm}  &  1.016  &  22.246  &  21.879 \hspace{0.3cm}  &  21.935 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.425 \hspace{0.05cm}  &  \hspace{0.05cm} -19.425 \hspace{0.3cm}  &  1.072  &  22.331  &  21.997 \hspace{0.3cm}  &  22.029 \hspace{0.05cm}  &  \hspace{0.05cm} -19.485 \hspace{0.3cm}  &  0.932  &  22.315  &  21.993 \hspace{0.3cm}  &  22.007 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.795 \hspace{0.05cm}  &  \hspace{0.05cm} -19.400 \hspace{0.3cm}  &  0.965  &  22.495  &  22.208 \hspace{0.3cm}  &  22.194 \hspace{0.05cm}  &  \hspace{0.05cm} -19.468 \hspace{0.3cm}  &  0.826  &  22.464  &  22.201 \hspace{0.3cm}  &  22.156 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.985 \hspace{0.05cm}  &  \hspace{0.05cm} -19.369 \hspace{0.3cm}  &  0.937  &  22.616  &  22.341 \hspace{0.3cm}  &  22.313 \hspace{0.05cm}  &  \hspace{0.05cm} -19.443 \hspace{0.3cm}  &  0.790  &  22.572  &  22.331 \hspace{0.3cm}  &  22.262 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.173 \hspace{0.05cm}  &  \hspace{0.05cm} -19.307 \hspace{0.3cm}  &  0.963  &  22.775  &  22.489 \hspace{0.3cm}  &  22.474 \hspace{0.05cm}  &  \hspace{0.05cm} -19.393 \hspace{0.3cm}  &  0.790  &  22.715  &  22.479 \hspace{0.3cm}  &  22.404 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.533 \hspace{0.05cm}  &  \hspace{0.05cm} - \hspace{0.3cm}  &  -  &  -  &  - \hspace{0.3cm}  &  - \hspace{0.05cm}  &  \hspace{0.05cm} -19.352 \hspace{0.3cm}  &  0.687  &  22.951  &  22.767 \hspace{0.3cm}  &  22.624 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.700 \hspace{0.05cm}  &  \hspace{0.05cm} - \hspace{0.3cm}  &  -  &  -  &  - \hspace{0.3cm}  &  - \hspace{0.05cm}  &  \hspace{0.05cm} -19.198 \hspace{0.3cm}  &  0.871  &  23.205  &  22.944 \hspace{0.3cm}  &  22.899 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.900 \hspace{0.05cm}  &  \hspace{0.05cm} - \hspace{0.3cm}  &  -  &  -  &  - \hspace{0.3cm}  &  - \hspace{0.05cm}  &  \hspace{0.05cm} -19.002 \hspace{0.3cm}  &  1.192  &  23.517  &  23.118 \hspace{0.3cm}  &  23.205 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 14.001 \hspace{0.05cm}  &  \hspace{0.05cm} - \hspace{0.3cm}  &  -  &  -  &  - \hspace{0.3cm}  &  - \hspace{0.05cm}  &  \hspace{0.05cm} -18.907 \hspace{0.3cm}  &  1.383  &  23.669  &  23.191 \hspace{0.3cm}  &  23.340 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 14.120 \hspace{0.05cm}  &  \hspace{0.05cm} - \hspace{0.3cm}  &  -  &  -  &  - \hspace{0.3cm}  &  - \hspace{0.05cm}  &  \hspace{0.05cm} -18.807 \hspace{0.3cm}  &  1.606  &  23.839  &  23.273 \hspace{0.3cm}  &  23.485 \hspace{0.05cm}  \\ 
\hline
\end{tabular}
} 
\end{center}
\end{table}
%-
\begin{table}
\begin{center}
\caption {Model D1M* at $B_{12}=100$} \label{tab:sigma_1}
\vskip 0.2cm
{\scriptsize
\begin{tabular}{ c | c c c c c | c c c c c }
\hline
&  &  &  $T$ = 1 MeV  &  &  &  &  &  $T$ = 5 MeV  &  &  \\ 
\hline
$\log\rho$ & $\log\tau$ & $\omega_c\tau$ & $\log\sigma$ & $\log\sigma_0$ & $\log\sigma_1$ & $\log\tau$ & $\omega_c\tau$ & $\log\sigma$ & $\log\sigma_0$ & $\log\sigma_1$ \\ 
\hline
\hspace{0.05cm} 11.825 \hspace{0.05cm}  &  \hspace{0.05cm} -19.402 \hspace{0.3cm}  &  1.349  &  22.199  &  21.745 \hspace{0.3cm}  &  21.878 \hspace{0.05cm}  &  \hspace{0.05cm} -19.461 \hspace{0.3cm}  &  1.178  &  22.196  &  21.744 \hspace{0.3cm}  &  21.868 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.001 \hspace{0.05cm}  &  \hspace{0.05cm} -19.423 \hspace{0.3cm}  &  1.234  &  22.214  &  21.810 \hspace{0.3cm}  &  21.903 \hspace{0.05cm}  &  \hspace{0.05cm} -19.480 \hspace{0.3cm}  &  1.081  &  22.208  &  21.807 \hspace{0.3cm}  &  21.892 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.167 \hspace{0.05cm}  &  \hspace{0.05cm} -19.426 \hspace{0.3cm}  &  1.172  &  22.250  &  21.872 \hspace{0.3cm}  &  21.943 \hspace{0.05cm}  &  \hspace{0.05cm} -19.484 \hspace{0.3cm}  &  1.025  &  22.241  &  21.870 \hspace{0.3cm}  &  21.929 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.425 \hspace{0.05cm}  &  \hspace{0.05cm} -19.424 \hspace{0.3cm}  &  1.081  &  22.325  &  21.986 \hspace{0.3cm}  &  22.022 \hspace{0.05cm}  &  \hspace{0.05cm} -19.485 \hspace{0.3cm}  &  0.941  &  22.309  &  21.983 \hspace{0.3cm}  &  22.002 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.795 \hspace{0.05cm}  &  \hspace{0.05cm} -19.401 \hspace{0.3cm}  &  0.972  &  22.487  &  22.196 \hspace{0.3cm}  &  22.185 \hspace{0.05cm}  &  \hspace{0.05cm} -19.468 \hspace{0.3cm}  &  0.833  &  22.456  &  22.189 \hspace{0.3cm}  &  22.148 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.985 \hspace{0.05cm}  &  \hspace{0.05cm} -19.366 \hspace{0.3cm}  &  0.953  &  22.609  &  22.327 \hspace{0.3cm}  &  22.307 \hspace{0.05cm}  &  \hspace{0.05cm} -19.440 \hspace{0.3cm}  &  0.804  &  22.566  &  22.318 \hspace{0.3cm}  &  22.256 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.173 \hspace{0.05cm}  &  \hspace{0.05cm} -19.307 \hspace{0.3cm}  &  0.977  &  22.764  &  22.472 \hspace{0.3cm}  &  22.463 \hspace{0.05cm}  &  \hspace{0.05cm} -19.392 \hspace{0.3cm}  &  0.802  &  22.705  &  22.462 \hspace{0.3cm}  &  22.395 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.533 \hspace{0.05cm}  &  \hspace{0.05cm} -19.069 \hspace{0.3cm}  &  1.340  &  23.203  &  22.755 \hspace{0.3cm}  &  22.883 \hspace{0.05cm}  &  \hspace{0.05cm} -19.206 \hspace{0.3cm}  &  0.978  &  23.083  &  22.771 \hspace{0.3cm}  &  22.779 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.700 \hspace{0.05cm}  &  \hspace{0.05cm} -18.891 \hspace{0.3cm}  &  1.810  &  23.476  &  22.845 \hspace{0.3cm}  &  23.103 \hspace{0.05cm}  &  \hspace{0.05cm} -19.077 \hspace{0.3cm}  &  1.178  &  23.304  &  22.907 \hspace{0.3cm}  &  22.992 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.900 \hspace{0.05cm}  &  \hspace{0.05cm} -18.666 \hspace{0.3cm}  &  2.668  &  23.814  &  22.903 \hspace{0.3cm}  &  23.330 \hspace{0.05cm}  &  \hspace{0.05cm} -18.930 \hspace{0.3cm}  &  1.451  &  23.561  &  23.051 \hspace{0.3cm}  &  23.223 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 14.001 \hspace{0.05cm}  &  \hspace{0.05cm} -18.541 \hspace{0.3cm}  &  3.324  &  23.996  &  22.915 \hspace{0.3cm}  &  23.437 \hspace{0.05cm}  &  \hspace{0.05cm} -18.855 \hspace{0.3cm}  &  1.613  &  23.692  &  23.121 \hspace{0.3cm}  &  23.337 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 14.068 \hspace{0.05cm}  &  \hspace{0.05cm} -18.460 \hspace{0.3cm}  &  3.828  &  24.119  &  22.924 \hspace{0.3cm}  &  23.507 \hspace{0.05cm}  &  \hspace{0.05cm} -18.809 \hspace{0.3cm}  &  1.714  &  23.779  &  23.170 \hspace{0.3cm}  &  23.411 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 14.120 \hspace{0.05cm}  &  \hspace{0.05cm} - \hspace{0.3cm}  &  -  &  -  &  - \hspace{0.3cm}  &  - \hspace{0.05cm}  &  \hspace{0.05cm} -18.735 \hspace{0.3cm}  &  1.947  &  23.889  &  23.195 \hspace{0.3cm}  &  23.491 \hspace{0.05cm}  \\ 
\hline
\end{tabular}
} 
\end{center}
\end{table}
%-
%\newpage
\begin{table}
\begin{center}
\caption {Model Bsk24 at $B_{12}=100$} \label{tab:sigma_1}
\vskip 0.2cm
{\scriptsize
\begin{tabular}{ c | c c c c c | c c c c c }
\hline
&  &  &  $T$ = 1 MeV  &  &  &  &  &  $T$ = 5 MeV  &  &  \\ 
\hline
$\log\rho$ & $\log\tau$ & $\omega_c\tau$ & $\log\sigma$ & $\log\sigma_0$ & $\log\sigma_1$ & $\log\tau$ & $\omega_c\tau$ & $\log\sigma$ & $\log\sigma_0$ & $\log\sigma_1$ \\ 
\hline
\hspace{0.05cm} 11.655 \hspace{0.05cm}  &  \hspace{0.05cm} -19.514 \hspace{0.3cm}  &  1.054  &  22.078  &  21.752 \hspace{0.3cm}  &  21.776 \hspace{0.05cm}  &  \hspace{0.05cm} -19.560 \hspace{0.3cm}  &  0.947  &  22.067  &  21.750 \hspace{0.3cm}  &  21.762 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 11.962 \hspace{0.05cm}  &  \hspace{0.05cm} -19.538 \hspace{0.3cm}  &  0.923  &  22.119  &  21.850 \hspace{0.3cm}  &  21.817 \hspace{0.05cm}  &  \hspace{0.05cm} -19.584 \hspace{0.3cm}  &  0.831  &  22.106  &  21.847 \hspace{0.3cm}  &  21.800 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.320 \hspace{0.05cm}  &  \hspace{0.05cm} -19.568 \hspace{0.3cm}  &  0.779  &  22.176  &  21.969 \hspace{0.3cm}  &  21.862 \hspace{0.05cm}  &  \hspace{0.05cm} -19.613 \hspace{0.3cm}  &  0.702  &  22.160  &  21.963 \hspace{0.3cm}  &  21.840 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.627 \hspace{0.05cm}  &  \hspace{0.05cm} -19.598 \hspace{0.3cm}  &  0.649  &  22.245  &  22.092 \hspace{0.3cm}  &  21.905 \hspace{0.05cm}  &  \hspace{0.05cm} -19.643 \hspace{0.3cm}  &  0.586  &  22.226  &  22.082 \hspace{0.3cm}  &  21.877 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.934 \hspace{0.05cm}  &  \hspace{0.05cm} -19.628 \hspace{0.3cm}  &  0.525  &  22.340  &  22.234 \hspace{0.3cm}  &  21.955 \hspace{0.05cm}  &  \hspace{0.05cm} -19.672 \hspace{0.3cm}  &  0.474  &  22.318  &  22.220 \hspace{0.3cm}  &  21.921 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.240 \hspace{0.05cm}  &  \hspace{0.05cm} -19.644 \hspace{0.3cm}  &  0.426  &  22.472  &  22.399 \hspace{0.3cm}  &  22.030 \hspace{0.05cm}  &  \hspace{0.05cm} -19.689 \hspace{0.3cm}  &  0.384  &  22.446  &  22.380 \hspace{0.3cm}  &  21.986 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.599 \hspace{0.05cm}  &  \hspace{0.05cm} -19.610 \hspace{0.3cm}  &  0.371  &  22.695  &  22.639 \hspace{0.3cm}  &  22.209 \hspace{0.05cm}  &  \hspace{0.05cm} -19.660 \hspace{0.3cm}  &  0.331  &  22.659  &  22.610 \hspace{0.3cm}  &  22.148 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.905 \hspace{0.05cm}  &  \hspace{0.05cm} -19.459 \hspace{0.3cm}  &  0.436  &  23.008  &  22.933 \hspace{0.3cm}  &  22.572 \hspace{0.05cm}  &  \hspace{0.05cm} -19.529 \hspace{0.3cm}  &  0.371  &  22.949  &  22.890 \hspace{0.3cm}  &  22.472 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 14.047 \hspace{0.05cm}  &  \hspace{0.05cm} -19.244 \hspace{0.3cm}  &  0.650  &  23.307  &  23.154 \hspace{0.3cm}  &  22.966 \hspace{0.05cm}  &  \hspace{0.05cm} -19.351 \hspace{0.3cm}  &  0.507  &  23.209  &  23.104 \hspace{0.3cm}  &  22.821 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 14.056 \hspace{0.05cm}  &  \hspace{0.05cm} -19.220 \hspace{0.3cm}  &  0.680  &  23.337  &  23.172 \hspace{0.3cm}  &  23.004 \hspace{0.05cm}  &  \hspace{0.05cm} -19.333 \hspace{0.3cm}  &  0.525  &  23.235  &  23.123 \hspace{0.3cm}  &  22.855 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 14.063 \hspace{0.05cm}  &  \hspace{0.05cm} -19.199 \hspace{0.3cm}  &  0.711  &  23.362  &  23.185 \hspace{0.3cm}  &  23.037 \hspace{0.05cm}  &  \hspace{0.05cm} -19.316 \hspace{0.3cm}  &  0.543  &  23.255  &  23.137 \hspace{0.3cm}  &  22.883 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 14.085 \hspace{0.05cm}  &  \hspace{0.05cm} -19.024 \hspace{0.3cm}  &  1.181  &  23.448  &  23.069 \hspace{0.3cm}  &  23.141 \hspace{0.05cm}  &  \hspace{0.05cm} -19.177 \hspace{0.3cm}  &  0.829  &  23.306  &  23.067 \hspace{0.3cm}  &  22.998 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 14.098 \hspace{0.05cm}  &  \hspace{0.05cm} -18.934 \hspace{0.3cm}  &  1.490  &  23.517  &  23.008 \hspace{0.3cm}  &  23.182 \hspace{0.05cm}  &  \hspace{0.05cm} -19.111 \hspace{0.3cm}  &  0.991  &  23.351  &  23.040 \hspace{0.3cm}  &  23.048 \hspace{0.05cm}  \\ 
\hline
\end{tabular}
} 
\end{center}
\end{table}
%-
\begin{table}
\begin{center}
\caption {Model Sly9 at $B_{12}=100$} \label{tab:sigma_1}
\vskip 0.2cm
{\scriptsize
\begin{tabular}{ c | c c c c c | c c c c c }
\hline
&  &  &  $T$ = 1 MeV  &  &  &  &  &  $T$ = 5 MeV  &  &  \\ 
\hline
$\log\rho$ & $\log\tau$ & $\omega_c\tau$ & $\log\sigma$ & $\log\sigma_0$ & $\log\sigma_1$ & $\log\tau$ & $\omega_c\tau$ & $\log\sigma$ & $\log\sigma_0$ & $\log\sigma_1$ \\ 
\hline
\hspace{0.05cm} 11.613 \hspace{0.05cm}  &  \hspace{0.05cm} -19.464 \hspace{0.3cm}  &  1.190  &  22.121  &  21.736 \hspace{0.3cm}  &  21.813 \hspace{0.05cm}  &  \hspace{0.05cm} -19.516 \hspace{0.3cm}  &  1.057  &  22.106  &  21.736 \hspace{0.3cm}  &  21.798 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.123 \hspace{0.05cm}  &  \hspace{0.05cm} -19.510 \hspace{0.3cm}  &  0.954  &  22.176  &  21.894 \hspace{0.3cm}  &  21.875 \hspace{0.05cm}  &  \hspace{0.05cm} -19.559 \hspace{0.3cm}  &  0.852  &  22.160  &  21.891 \hspace{0.3cm}  &  21.855 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.623 \hspace{0.05cm}  &  \hspace{0.05cm} -19.555 \hspace{0.3cm}  &  0.738  &  22.263  &  22.073 \hspace{0.3cm}  &  21.942 \hspace{0.05cm}  &  \hspace{0.05cm} -19.603 \hspace{0.3cm}  &  0.661  &  22.243  &  22.064 \hspace{0.3cm}  &  21.915 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 12.891 \hspace{0.05cm}  &  \hspace{0.05cm} -19.576 \hspace{0.3cm}  &  0.632  &  22.334  &  22.188 \hspace{0.3cm}  &  21.990 \hspace{0.05cm}  &  \hspace{0.05cm} -19.624 \hspace{0.3cm}  &  0.566  &  22.312  &  22.176 \hspace{0.3cm}  &  21.956 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.091 \hspace{0.05cm}  &  \hspace{0.05cm} -19.582 \hspace{0.3cm}  &  0.569  &  22.408  &  22.285 \hspace{0.3cm}  &  22.041 \hspace{0.05cm}  &  \hspace{0.05cm} -19.631 \hspace{0.3cm}  &  0.508  &  22.382  &  22.270 \hspace{0.3cm}  &  22.002 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.191 \hspace{0.05cm}  &  \hspace{0.05cm} -19.580 \hspace{0.3cm}  &  0.545  &  22.452  &  22.339 \hspace{0.3cm}  &  22.076 \hspace{0.05cm}  &  \hspace{0.05cm} -19.630 \hspace{0.3cm}  &  0.486  &  22.424  &  22.321 \hspace{0.3cm}  &  22.032 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.291 \hspace{0.05cm}  &  \hspace{0.05cm} -19.571 \hspace{0.3cm}  &  0.529  &  22.504  &  22.397 \hspace{0.3cm}  &  22.121 \hspace{0.05cm}  &  \hspace{0.05cm} -19.623 \hspace{0.3cm}  &  0.469  &  22.473  &  22.377 \hspace{0.3cm}  &  22.072 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.393 \hspace{0.05cm}  &  \hspace{0.05cm} -19.555 \hspace{0.3cm}  &  0.520  &  22.565  &  22.461 \hspace{0.3cm}  &  22.178 \hspace{0.05cm}  &  \hspace{0.05cm} -19.610 \hspace{0.3cm}  &  0.459  &  22.530  &  22.438 \hspace{0.3cm}  &  22.123 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.491 \hspace{0.05cm}  &  \hspace{0.05cm} -19.530 \hspace{0.3cm}  &  0.524  &  22.634  &  22.529 \hspace{0.3cm}  &  22.248 \hspace{0.05cm}  &  \hspace{0.05cm} -19.589 \hspace{0.3cm}  &  0.457  &  22.594  &  22.503 \hspace{0.3cm}  &  22.185 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.591 \hspace{0.05cm}  &  \hspace{0.05cm} -19.493 \hspace{0.3cm}  &  0.542  &  22.717  &  22.605 \hspace{0.3cm}  &  22.340 \hspace{0.05cm}  &  \hspace{0.05cm} -19.558 \hspace{0.3cm}  &  0.467  &  22.670  &  22.576 \hspace{0.3cm}  &  22.265 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.691 \hspace{0.05cm}  &  \hspace{0.05cm} -19.442 \hspace{0.3cm}  &  0.578  &  22.813  &  22.688 \hspace{0.3cm}  &  22.450 \hspace{0.05cm}  &  \hspace{0.05cm} -19.516 \hspace{0.3cm}  &  0.488  &  22.756  &  22.655 \hspace{0.3cm}  &  22.362 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.791 \hspace{0.05cm}  &  \hspace{0.05cm} -19.377 \hspace{0.3cm}  &  0.639  &  22.922  &  22.774 \hspace{0.3cm}  &  22.579 \hspace{0.05cm}  &  \hspace{0.05cm} -19.462 \hspace{0.3cm}  &  0.525  &  22.852  &  22.738 \hspace{0.3cm}  &  22.475 \hspace{0.05cm}  \\ 
\hspace{0.05cm} 13.809 \hspace{0.05cm}  &  \hspace{0.05cm} -19.364 \hspace{0.3cm}  &  0.653  &  22.943  &  22.789 \hspace{0.3cm}  &  22.604 \hspace{0.05cm}  &  \hspace{0.05cm} -19.451 \hspace{0.3cm}  &  0.534  &  22.871  &  22.753 \hspace{0.3cm}  &  22.497 \hspace{0.05cm}  \\ 
\hline
\end{tabular}
} 
\end{center}
\end{table}
%\end{document}

